Faster Unbalanced Optimal Transport: Translation invariant Sinkhorn and 1-D Frank-Wolfe

Unbalanced optimal transport (UOT) extends optimal transport (OT) to take into account mass variations to compare distributions. This is crucial to make OT successful in ML applications, making it robust to data normalization and outliers. The baseline algorithm is Sinkhorn, but its convergence speed might be significantly slower for UOT than for OT. In this work, we identify the cause for this deficiency, namely the lack of a global normalization of the iterates, which equivalently corresponds to a translation of the dual OT potentials. Our first contribution leverages this idea to develop a provably accelerated Sinkhorn algorithm (coined 'translation invariant Sinkhorn') for UOT, bridging the computational gap with OT. Our second contribution focusses on 1-D UOT and proposes a Frank-Wolfe solver applied to this translation invariant formulation. The linear oracle of each steps amounts to solving a 1-D OT problems, resulting in a linear time complexity per iteration. Our last contribution extends this method to the computation of UOT barycenter of 1-D measures. Numerical simulations showcase the convergence speed improvement brought by these three approaches.

==> sections/experiment.tex <==
% !TEX root = ../AISTATS-Unbalanced.tex


\section{Experiments}
\label{sec-xp}

\subsection{Convergence of Sinkhorn}

In this section we track the convergence of the dual potentials of the Sinkhorn algorithm compared to our proposal where an optimal translation is computed at each loop using Equations~\eqref{eq-sink-with-trans-1} and~\eqref{eq-sink-with-trans-2}.

Recall that the classical Sinkhorn algorithm has a geometric convergence rate of $(1 + \tfrac{\epsilon}{\rho})^{-1}$.
%
For this reason we plot a first experiment where the ratio $\epsilon / \rho$ is fixed, and we update $\epsilon_t = t * \epsilon$ and $\rho_t = t * \rho$ for $t\in[10, 1, 0.1, 0.01]$.
%
We display the experiment on Figure~\ref{fig-sinkhorn-ratio-fixed}.
%
Note that all dotted lines are parallel, showing that the ratio $\epsilon / \rho$ being fixed yields the same convergence for the classic Sinkhorn algorithm, independently of the scaling.
%
Compared to this, the adjunction of translations provides a convergence at least as fast as the standard algorithm, but which accelerates as the scaling increases, thus highlighting the benefits of translating the potentials in the iterations.

\begin{figure}[H]
	\centering
	\includegraphics[width=0.45\textwidth]{sections/figures/plot_sinkhorn_ratio_fixed.png}
	\caption{Convergence of the dual potential $\f$ towards the optimal $\f^*$ w.r.t $\norm{\cdot}_\infty$. Each color corresponds to a scaling $t$ of $(\epsilon_t, \rho_t)$. The convergence for Sinkhorn are plotted as dotted lines, and our proposal with solid ones.}
	\label{fig-sinkhorn-ratio-fixed}
\end{figure}

We display in Figures~\ref{fig-sinkhorn-eps-fixed} and~\ref{fig-sinkhorn-rho-fixed} the plots of convergence when respectively $\epsilon$ and $\rho$ are fixed.
%
In those cases the ratio $\epsilon / \rho$ is not fixed, hence the change of slopes for the dotted.
%
We see that in both settings the homogeneous algorithm yields a convergence which is at least as fast as its standard counterpart, thus highlighting its benefits.
%
What remains an open question is the rate of convergence for the homogeneous algorithm, and why the first iterations of both algorithm seem very close w.r.t. $\norm{\cdot-\f^*}_\infty$.

\begin{figure}[!htb]
	\begin{minipage}{0.45\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{sections/figures/plot_sinkhorn_eps_fixed.png}
		\caption{Value of $\norm{\f_t - \f^*}_\infty$ for $\epsilon=5.10^{-3}$ and $\rho\in\{0.1, 1, 10, 100\}$ for the standard Sinkhorn algorithm and the homogeneous version.}\label{fig-sinkhorn-eps-fixed}
	\end{minipage}\hfill
	\begin{minipage}{0.45\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{sections/figures/plot_sinkhorn_rho_fixed.png}
		\caption{Value of $\norm{\f_t - \f^*}_\infty$ for $\rho=5$ and $\epsilon\in\{0.001, 0.01, 0.1, 1\}$ for the standard Sinkhorn algorithm and the homogeneous version.}\label{fig-sinkhorn-rho-fixed}
	\end{minipage}
\end{figure}

Lastly, we compute the Anderson acceleration~\cite{anderson1965iterative} for the standard and homogeneous Sinkhorn algorithm.
%
\todo{Explain the acceleration.}
%
The goal is to verify if the acceleration benefits from this proposed algorithm, and if the accelerated Sinkhorn is faster than the homogeneous algorithm.
%
As displayed by Figure~\ref{fig-sinkhorn-anderson}, we see that Sinkhorn accelerated with Anderson extrapolation is slower than the homogeneous algorithm, and that accelerate this algorithm yields a faster convergence.

\begin{figure}[H]
	\centering
	\includegraphics[width=0.45\textwidth]{sections/figures/plot_sinkhorn_with_anderson.png}
	\caption{Convergence of the dual potential $\f$ towards the optimal $\f^*$ w.r.t $\norm{\cdot}_\infty$ for $\epsilon=0.01$ and $\rho=10$.}
	\label{fig-sinkhorn-anderson}
\end{figure}


\subsection{Benchmark of 1D Frank-Wolfe}

\subsection{Unbalanced Barycenters in 1D}

==> sections/translations.tex <==
% !TEX root = ../AISTATS-Unbalanced.tex


\section{Consequences of the dual invariance to translations}
\label{sec-transl}

%\subsection{Closed form in KL setting}
%
%In this section we present properties and consequences of seeking a dual formulation invariant to translation. We focus on the setting of $\KL$ divergence where $\phi_i(x) = \rho_i(x\log x - x + 1)$, with $(\rho_1,\rho_2)>0$.
%%
%In that case the optimal translation admits a closed form.
%
%\begin{prop}
%	\label{prop-kl-opt-trans}
%	Consider the KL setting $\phi_i(x) = \rho_i(x\log x - x + 1)$. Then the optimal $\la^*$ from Proposition~\ref{prop-equiv-mass-trans} is expressed as
%	\eql{\label{eq-opt-trans-kl}
%		\la^* = \tfrac{\rho_1\rho_2}{\rho_1 + \rho_2} \log\Big[\frac{\dotp{\al}{e^{-\f / \rho_1}}}{ \dotp{\be}{e^{-\g / \rho_2}}}\Big].
%	}
%\end{prop}
%
%Thus the normalization step in the FW is particularly simple, and can be stabilized via a logsumexp reduction.
%%
%An important consequence of Proposition~\ref{prop-kl-opt-trans} is a new dual formulation in the KL setting which is new to the best of our knowledge.
%
%\begin{prop}
%	Setting $\tau_1=\rho_1/(\rho_1+\rho_2)$ and $\tau_2=\rho_2/(\rho_1+\rho_2)$, the dual formulation is equivalent to
%\begin{align}
%	&\UOT(\al,\be) =  \rho_1 m(\al) + \rho_2 m(\be)\nonumber \\
%	&+\sup_{\f\oplus\g\leq\C}- (\rho_1 + \rho_2)\Big(\dotp{\al}{ e^{-\f / \rho_1} }\Big)^{\tau_1} \Big(\dotp{\be}{ e^{-\g / \rho_2} }\Big)^{\tau_2}.\label{eq-dual-form-hell}
%\end{align}
%
%In particular when $\rho_1 = \rho_2=\rho$,
%\begin{align*}
%	\UOT&(\al,\be) = \rho (m(\al) +  m(\be))\\ 
%	&+ \sup_{\f\oplus\g\leq\C} - 2\rho\sqrt{   \dotp{\al}{ e^{-\f / \rho_1} } \cdot \dotp{\be}{ e^{-\g / \rho_2} }   }.
%\end{align*}
%
%\end{prop}


\subsection{Accelerating Sinkhorn}

Optimizing the constant is an ingredient which we prove in this section to significantly accelerate the Sinkhorn algorithm.
\todo{}
%
We focus in this section on the KL setting, and introduce notations from~\cite{bibid}.
%
Recall that the Sinkhorn algorithm optimizes the dual of entropically regularized UOT which reads
\begin{align}\label{eq-entropic-uot}
	\UOT_\epsilon(\al,\be) \triangleq \umax{(\f,\g)} &\dotp{\al}{-\rho_1(e^{-\f / \rho_1} - 1)}\\
	 + &\dotp{\be}{-\rho_2(e^{-\g / \rho_2} - 1)}\\
	  - &\epsilon\dotp{\al\otimes\be}{e^{\tfrac{\f\oplus\g-\C}{\epsilon}} - 1}.
\end{align}

The Sinkhorn algorithm updates $\f$ and $\g$ alternatively until convergence.
%
In the KL setting, it is proved in~\cite{bibid} that the Sinkhorn algorithm reads for any initialization $\f_0$
\begin{align*}
	\g_{t+1}(y) &= \aprox_{\rho_1}(\Smin{\al}{\epsilon}(\C(\cdot,y) - \f_{t})),\\
	\f_{t+1}(x) &= \aprox_{\rho_2}(\Smin{\be}{\epsilon}(\C(x,\cdot) - \g_{t+1})),
\end{align*}
where the softmin $\Smin{}{}$ and the anisotropic proximity operator $\aprox$ read $\Smin{\al}{\epsilon}(\f) \triangleq -\epsilon\log\dotp{\al}{e^{-\f / \epsilon}}$, and $\aprox_\rho(\f) \triangleq \tfrac{\rho}{\rho + \epsilon} \f$.

Both operators are respectively $1$-contractive and $(1+\tfrac{\epsilon}{\rho})^{-1}$-contractive for the uniform norm $\norm{\cdot}_\infty$. We introduce an operator which applies the optimal translation from Proposition~\ref{prop-kl-opt-trans}, noted $\la^*(\f,\g)$. It reads
\begin{align}
	&T_1(\f,\g)\triangleq \f + \la^*(\f,\g), \\ 
	&T_2(\f,\g)\triangleq \g + \la^*(\f,\g).
\end{align}

We propose to add an extra step in the Sinkhorn algorithm by translating after applying the operator $\aprox\circ\Smin{}{}$, which now read
\begin{gather}
\g_{t+1}(y) = \aprox_{\rho_1}\bigg(\Smin{\al}{\epsilon}\big(\C(\cdot,y) - \f_{t} - T_1(\f_{t}, \g_{t})\big)\bigg),\label{eq-sink-with-trans-1}\\
\f_{t+1}(x) = \aprox_{\rho_2}\bigg(\Smin{\be}{\epsilon}\big(\C(x,\cdot) - \g_{t+1} + T_2(\f_{t+1}, \g_{t+1})\big)\bigg).\label{eq-sink-with-trans-2}
\end{gather}

\todo{Move it in a first section on Sinkhorn and alternate descent}
This sequence of updates operates an alternate dual ascent on the following formulation
\begin{align}
	\sup_{\f,\g,\la} \dotp{\al}{-\rho_1(e^{\tfrac{\f-\la}{\rho_1}} - 1)} + \dotp{\be}{-\rho_2(e^{\tfrac{\g+\la}{\rho_2}} - 1)}
	-\epsilon\dotp{\al\otimes\be}{e^{\tfrac{\f\oplus\g - \C}{\epsilon}} - 1}. \label{eq-dual-form-with-trans}
\end{align}

Note that an alternate descent on the above formulation is not equivalent to operate an alternate descent on Formulation~\eqref{eq-dual-form-hell}.
%
Indeed, when $\rho_1=\rho_2=\rho$, the first order condition of Formulation~\eqref{eq-dual-form-hell} w.r.t. $\f$ for fixed $\g_t$ reads
\begin{align}
	e^{\f / \epsilon}\cdot\dotp{\be}{e^{\tfrac{\g_t - \C}{\epsilon}}} = e^{-\f / \rho}\cdot\sqrt{\frac{ \dotp{\be}{e^{-\g_t / \rho}} }{ \dotp{\al}{e^{-\f / \rho}} }}.\label{eq-optim-sink-v1}
\end{align}

Concerning Formulation~\eqref{eq-dual-form-with-trans}, the optimality on $\f$ for fixed $(\g_t,\la_t)$ where $\la_t=\la^*(\f_t,\g_t)$ reads
\begin{align}
	e^{\f / \epsilon}\cdot\dotp{\be}{e^{\tfrac{\g_t - \C}{\epsilon}}} = e^{\tfrac{-\f-\la_t}{\rho}} = e^{-\f / \rho}\cdot\sqrt{\frac{ \dotp{\be}{e^{-\g_t / \rho}} }{ \dotp{\al}{e^{-\f_t / \rho}} }}.\label{eq-optim-sink-v2}
\end{align}
Note that while the optimality Equation~\eqref{eq-optim-sink-v1} is an equation which does not admit a closed form due to the dependence in $\f$ of the integral $\dotp{\al}{e^{-\f / \rho}}$, Equation~\eqref{eq-optim-sink-v2} admits a closed form for $\f$ because it uses the previously computed potential $\f_t$.

We provide experiments in Section~\ref{sec-xp}. At the moment we have no proof that the rate of convergence is better using this algorithm, but we observe experimentally that this algorithm converges at least as fast as the standard Sinkhorn algorithm.


























%We prove now that $T_1$ and $T_2$ are both contractions for $\norm{\cdot}_\infty$, thus they will accelerate the above Sinkhorn algorithm.
%
%\begin{prop}
%	The operators $T_1$ and $T_2$ are respectively $(1 + \tfrac{\rho_1}{\rho_2})^{-1}$ and $(1 + \tfrac{\rho_2}{\rho_1})^{-1}$-contractive, in the sense that for any continuous function $\h$, one has
%	\begin{align*}
%		\norm{T_1(\f,\h) - T_1(\g,\h)}_\infty &\leq \frac{\rho_2}{\rho_1 + \rho_2}\norm{\f - \g}_\infty,\\
%		\norm{T_2(\h,\f) - T_2(\h,\g)}_\infty &\leq \frac{\rho_1}{\rho_1 + \rho_2}\norm{\f - \g}_\infty.
%	\end{align*}
%\end{prop}
%\begin{proof}
%	We prove the result for the first argument, the proof for the second being the same.
%	%
%	Take functions $\f,\g,\h$, and study the difference $T_1(\f,\h) - T_1(\g,\h)$.
%	%
%	Reusing Equation~\eqref{eq-opt-trans-kl}, one has
%	\begin{align*}
%		T_1(\f,\h) - T_1(\g,\h) &= \tfrac{\rho_1\rho_2}{\rho_1 + \rho_2}\Big[\log\dotp{\al}{e^{-\f / \rho_1}} - \log\dotp{\al}{e^{-\g / \rho_1}}\Big]\\
%		&= \tfrac{\rho_2}{\rho_1 + \rho_2}\Big[\rho_1\log\dotp{\al}{e^{-\f / \rho_1}} - \rho_1\log\dotp{\al}{e^{-\g / \rho_1}}\Big]\\
%		&= \tfrac{\rho_2}{\rho_1 + \rho_2}\Big[\Smin{\al}{\rho_1}(\g) - \Smin{\al}{\rho_1}(\f)  \Big].
%	\end{align*}
%	Since the Softmin is $1$-contractive, we have
%	\begin{align*}
%		\norm{T_1(\f,\h) - T_1(\g,\h)}_\infty \leq \tfrac{\rho_2}{\rho_1 + \rho_2} \norm{\Smin{\al}{\rho_1}(\f) - \Smin{\al}{\rho_1}(\g)}_\infty
%		\leq \tfrac{\rho_2}{\rho_1 + \rho_2}\norm{\f - \g}_\infty,
%	\end{align*}
%	which ends the proof.
%\end{proof}
%
%
%Due to the strict convexity in $(\f,\g)$ of Problem~\eqref{eq-entropic-uot}, the optimal $(\f,\g)$ is unique, and the proposed algorithm output the same potentials as the standard Sinkhorn algorithm.
%%
%Though, the contractance rates of both algorithm differ, which has an impact on the geometric convergence of potentials.
%%
%The standard algorithm has a contractance rate of $\tau= (1 + \tfrac{\epsilon}{\rho_1})^{-1}(1 + \tfrac{\epsilon}{\rho_2})^{-1}$ after a whole loop.
%%
%The issue is that $\tau$ quickly approaches $1$ when $\epsilon\rightarrow 0$ or when $(\rho_1,\rho_2)$ become large compared to $\epsilon$.
%%
%In those settings, the standard Sinkhorn algorithm converges very slowly.
%
%Compared to this, adding the translations yields a rate $\kappa = \tau\cdot (1 + \tfrac{\rho_2}{\rho_1})^{-1}(1 + \tfrac{\rho_1}{\rho_2})^{-1}$. 
%%
%Since $(1 + \tfrac{\rho_2}{\rho_1})^{-1}+(1 + \tfrac{\rho_1}{\rho_2})^{-1}=1$ and for $x\in[0,1]$ one has $x(1-x)\leq 1/4$. 
%%
%Thus one has $\kappa\leq \tau / 4$, which provides a significantly better rate on the geometric convergence of potentials, even when $\tau\simeq 1$.
%
%A last important remark is that computing the translation~\eqref{eq-opt-trans-kl} does not involve the cost matrix, and has a $O(N)$ complexity where $N$ is the number of samples. 
%%
%Thus this extra step has little impact on the total computational time which is dominated by the $O(N^2)$ cost to compute the Softmin.
